Gravitational Lensing in Standard and Alternative Cosmologies

This thesis contributes to the field of gravitational lensing (GL) and observational cosmology. We discuss the use of gravitational lensing as a tool in search of exotic objects in the Universe. In the next chapter the concordance of an alternative cosmological model with the current gravitational lensing observations is explored and also a non-minimally coupled effective gravity theory that supports non-topological solitonic solutions is considered. In the last chapter we study propagation of light in strong gravitational field. Using geometrical optics approach we show that massless particles with spin deviate from the geodesic motion. We demonstrate that the velocity of photon propagating in a Kerr black hole background remains subluminal.

==> chapter3/references.tex <==
\bibitem{motho}M. S. Morris \& K. S. Thorne, Am. J. Phys. {\bf 56},
395 (1988).

\bibitem{wh}L. A. Anchordoqui, S. E. Perez Bergliaffa \& D.
F. Torres, Phys. Rev. D {\bf 55}, 5226 (1997); A. DeBenedictis and
A. Das [gr-qc/0009072]; S. E. Perez Bergliaffa and K. E. Hibberd,
Phys. Rev. D {\bf 62}, 044045 (2000); C. Barcelo and M. Visser,
Nucl. Phys. {\bf B584}, 415 (2000); L. A. Anchordoqui and S. E.
Perez Bergliaffa, Phys. Rev. D {\bf 62}, 067502 (2000); D.
Hochberg, A. Popov, and S. V. Sushkov, Phys. Rev. Lett. {\bf 78},
2050 (1997); S. Kim and H. Lee, Phys. Lett. B {\bf 458}, 245
(1999); S. Krasnikov, Phys. Rev. D {\bf 62}, 084028 (2000); D.
Hochberg and M. Visser, Phys. Rev. D {\bf 56}, 4745 (1997).

\bibitem{VISSER-BOOK}M. Visser, {\it Lorentzian Wormholes}
(AIP, New York, 1996).
                          \bibitem{h-v}D. Hochberg and M. Visser, Phys. Rev. Lett. {\bf 81}, 746 (1998).

\bibitem{h-v2}D. Hochberg and M. Visser, Phys. Rev. D{\bf 58}, 044021
(1998).

\bibitem{last-visser}C. Barcel\'o and M. Visser, Phys. Lett. B {\bf 466},
127 (1999); M. Visser, talk at the Marcel Grossman Meeting, Rome,
July 2000; C. Barcelo and M. Visser, Class. Quant. Grav. {\bf 17},
3843, (2000).

\bibitem{JAMMER}M. Jammer, {\it Concepts of mass} (Dover, New York, 1997).

\bibitem{BONDI}H. Bondi, Rev. Mod. Phys. {\bf 29}, 423 (1957).

\bibitem{cube}M. Visser, Phys. Rev. D{\bf 39}, 3182 (1989); Nucl.
Phys. B{\bf 328}, 203 (1989).

\bibitem{ROMAN} T. Roman, Phys. Rev. D{\bf 47}, 1370 (1993).

\bibitem{Mann} R. B. Mann, Class. Quant. Grav. {\bf 14},  2927 (1997).

            \bibitem{swkim}S.-W. Kim and Y. M. Cho, in {\it Evolution of the Universe
and its Observational Quest} (Universal Academy Press, Inc. and
Yamada Science Foundation, 1994), p. 353.

\bibitem{cramer}J. Cramer, R. Forward, M. Morris, M. Visser, G. Benford,
and G. Landis, Phys. Rev. D {\bf 51}, 3117 (1995).

\bibitem{diego-grbwh}D. F. Torres, G. E. Romero, and L. A. Anchordoqui,
Phys. Rev. D {\bf 58}, 123001 (1998); D. F. Torres, G. E. Romero,
and L. A. Anchordoqui, {\it (Honorable Mention, Gravity Foundation
Research Awards 1998)}, Mod. Phys. Lett. {\bf A13}, 1575 (1998).

\bibitem{doqui}L. Anchordoqui, G. E. Romero, D. F. Torres, and I. Andruchow,
Mod. Phys. Lett. {\bf A14}, 791 (1999).

\bibitem{rom}G. E. Romero, D. F. Torres, I. Andruchow, L. A. Anchordoqui,
and B. Link, Mon. Not. R. Astron. Soc. {\bf 308}, 799 (1999).

\bibitem{Zwart}S. F. Portegies Zwart, C-H. Lee, and H.K. Lee, \apj
{\bf 520}, 666 (1999).

\bibitem{macro}M. Safonova, D. F. Torres, and
G. E. Romero, Mod.\ Phys.\ Lett.\ {\bf A16}, 153 (2001).

\bibitem{eiroa}E. Eiroa, G. E. Romero, and D. F. Torres, {\it Chromaticity
effects in wormhole microlensing}, Mod. Phys. Lett. A (to be
published, 2001), gr-qc/0104076

\bibitem{Schneider} P. Schneider, J. Ehlers, and E. E. Falco, {\it Gravitational Lenses}
(Springer-Verlag Berlin Heidelberg New York, 1992).

\bibitem{Narayan} R. Narayan and M. Bartelmann, in {\it Formation
of Structure in the Universe}, edited by A. Dekel and J. P.
Ostriker (Cambridge, Cambridge University Press, 1999), p.360.

\bibitem{Kayser1986} R. Kayser, S. Refsdal, and R. Stabell, Astron. Astrophys.
{\bf 166}, 36 (1986).

\bibitem{Schneider2} P. Schneider and A. Weiss, Astron. Astrophys.
{\bf 171}, 49 (1987).

\bibitem{Osterbrock1976}D. E. Osterbrock, A. T. Koski, and
M. M. Phillips, \apj {\bf 206}, 898 (1976).

\bibitem{blan} R. D. Blanford and A. Levinson, \apj {\bf 441}, 79 (1995).

\bibitem{Schramm1987}T. Schramm and R. Kayser, Astron. Astrophys. {\bf 174},
361 (1987).

\bibitem{sazhin1}M. V. Sazhin and A. F. Zakharov, Usp. Fiz. Nauk
[Sov. Phys.--Usp], {\bf 168}, 1041 (1998).
        \bibitem{nec} D. Hochberg, A. Popov, and S. V. Sushkov, Phys. Rev.
              Lett. {\bf 78}, 2050 (1997);
S. Kim and H. Lee, Phys. Lett. {\bf B458}, 245 (1999); S. Hayward,
Int. J. Mod. Phys. {\bf D8}, 373 (1999); S. Krasnikov, Phys. Rev.
{\bf D62}, 084028 (2000); L.A. Anchordoqui, S. E. Perez Bergliaffa
and D. F. Torres, Phys. Rev. {\bf D55}, 5226 (1997); C. Barcel\'o
and M. Visser, Phys. Lett. {\bf B466}, 127 (1999); Class. Quant.
Grav. {\bf 17}, 3843 (2000); A. DeBenedictis and A. Das,
[gr-qc/0009072].

\bibitem{JAMMER} M. Jammer, {\it Concepts of mass}, (Dover, New
York, 1997).
        \bibitem{BONDI} H. Bondi, Rev. Mod. Phys. {\bf 29}, 423 (1957).

\bibitem{PIRAN-0} T. Piran, Gen. Rel. Grav. {\bf 29}, 1363 (1997).

\bib\bibitem{BONDI} H. Bondi, Rev. Mod. Phys. {\bf 29}, 423 (1957).

\bibitem{PIRAN-0} T. Piran, Gen. Rel. Grav. {\bf 29}, 1363 (1997).

\bibitem{MANN} R. Mann, Class. Quant. Grav. {\bf 14}, 2927 (1997).

\bibitem{wormhole-papers} M. S. Morris and
K. S. Thorne, Am. J. Phys. {\bf 56}, 395 (1987); M. Morris, K.
Thorne and U. Yurtserver, Phys. Rev. Lett. {\bf 61}, 1446 (1988).

\bibitem{karsan} S. Kar, D. Sahdev, and B. Bhawal, Phys. Rev. {\bf
                             D49}, 853 (1994).
                             S. E. Perez Bergliaffa and K. E. Hibberd, Phys.
                    Rev. {\bf D62}, 044045 (2000); G. Lambiase, S.
                    Capozziello, D. F. Torres, and L. A.
                    Anchordoqui, Submitted 2001.

\bibitem{e} L. A. Anchordoqui, S. Capozziello, G. Lambiase
and D. F. Torres, Mod. Phys. Lett. {\bf A15}, 2219 (2000).


\bibitem{cramer} J. Cramer, R. Forward, M. Morris, M. Visser, G.
                 Benford, and G. Landis, Phys. Rev. {\bf D51},
                 3117 (1995).
      \bibitem{diego-grwh} D. F. Torres, G. Romero, L. Anchordoqui, Phys. Rev.
                {\bf D58}, 123001 (1998); Mod. Phys. Lett. {\bf A13},
                1575 (1998). L. Anchordoqui, G. E. Romero, D. F. Torres and I. Andruchow,
                Mod. Phys. Lett. {\bf A14}, 791 (1999);
                G. E. Romero, D. F. Torres, I. Andruchow, L. A.
                Anchordoqui and B. Link, Mon. Not. R. Ast. Soc. {\bf 308}, 799 (1999).

\bibitem{VISSER-HUBBLE} M. Visser, Phys. Rev. {\bf D56}, 7578 (1997);
Science {\bf 276}, 88 (1997).

\bibitem{US} M. Safonova, D. F. Torres and G. E. Romero, in
preparation (2001).

\bibitem{1} W. H. Press, S. A. Teukolsky, W. T. Vetterling
\& B. P. Flannery {\it Numerical Recipes in FORTRAN}, $2^{{\rm
nd}}$ edition (Cambridge University Press, Cambridge, England,
1992).

\bibitem{2}P. Schneider, J. Ehlers \& E. E. Falco,
{\it Gravitational lenses} (Springer-Verlag, Berlin, 1992).

\bibitem{5}J. A. Tyson, Astron. J {\bf 96}, 1 (1988).

\bibitem{3} M. Bartelmann, A.
Huss, J. M. Colberg, A. Jenkins \& F. R. Pearce, {\it Large Scale
Structure:  Tracks and Traces}. Proceedings of the 12th Potsdam
Cosmology Workshop, held in Potsdam, September 15th to 19th, 1997.
Eds. V. Mueller, S. Gottloeber, J.P. Muecket, J. Wambsganss
World Scientific 1998, p. 321-324.

\bibitem{4}N. A. Bahcall and R. M. Soneira, Astrophys. Lett. {\bf 258}, L17
(1982).

\bibitem{6} A. R. Cooray, J. M. Quashnock, and M. C. Miller, Astrophys. J.
{\bf 511}, L562 (1999).

\bibitem{ULT} E. E. Flanagan and R. M. Wald, Phys. Rev. {\bf D54},
6233 (1996); M. Visser and C. Barcelo, [gr-qc/000109].






==> chapter4/ch4_3.tex <==
\subsection{Linear Coasting Cosmology}

After the discovery of the first multipy imaged quasars, gravitational
arcs and arclets, gravitational lensing has rapidly become one of the 
most promising tools for cosmology. It is now well known that gravitational
lensing is a useful probe of the geometry of the universe. With the rapid
growth of the number of lensed systems, proposals were made to apply the
statistical analysis to the samples of lenses in order to extract the
cosmological parameters. The use of gravitational lensing statistics as a
cosmological tool was first considered in detail by Turner et al. \cite{TOG}
and Fukugita et al \cite{fukugita}. More recently, Kochanek \cite{K96} and
Falco et al \cite{Falco98} have laid the groundwork for using gravitational
lensing statistics for the detailed analysis of the extragalactic surveys. It
has been pointed out \cite{fukugita,turner90} that the expected frequency of
multiple imaging lensing events for high-redshift sources is sensitive to a
cosmology. In view of the succesfull results of the above mentioned works
\cite{annu,abha}, it was tempting to use this test to constrain the power
index of the scale factor of a general power law cosmology, $ a(t) \propto
t^{\alpha}$. Expected number of lens systems depends upon the index $\alpha$ 
through the angular diameter distances. By varying $\alpha$, the number of 
lenses changes and on comparison with the observations gives us constraints on
$\alpha$. We find that the value of $\alpha=1$, corresponding to the coasting
cosmology, is in corcordance with the number of observed lenses in a considered
sample.  

We consider a general power law cosmology with the scale factor
given in terms of two parameters
\be
a(t)=B\fr{c}{H_0}\left(\fr{t}{t_0}\right)^{\a}\,\,,
\label{eq:ansatz}
\end{equation}
for an open FRW metric. However, the light propagates through the
inhomogeneous rather than the averaged smooth spacetime; the light ray feels
the local metric which deviates from the smooth FRW metric---FRW metric
excludes gravitational lensing in principle. We may assume, however, that the
relation between the affine distance of the null geodesic and the redshift of
the source object in a clumpy universe is the same as in the FRW cosmology.
This maybe regarded as a mathematical expression of the assumption that the
universe is described by FRW geometry on large scales (for the metric
see Eq.~\ref{eq:frw}).

\vspace{-0.5in}
\subsubsection{Dimensionless Hubble parameter}

The expansion rate of the universe is described by a Hubble parameter, $H =
\dot{a}/a$. Using (\ref{eq:ansatz}), \be
H(t)=\fr{\a}{t}\,\,.
\label{eq:exact}
\end{equation}
The {\it present} expansion rate of the universe is defined by a Hubble {\it
constant}, equal in our model to $H_0=\a/t_0$ (here and subsequently the
subscript 0 on a parameter refers to its present value). With the usual
definition of the redshift $z$
\be
\frac{a_0(z)}{a(z)} = 1+z
\label{eq:redshift}
\end{equation}
we obtain $t_0/t = (1+z)^{1/\a}$ and
\be 
H(z) = H_0 (1+z)^{1/\a}\,\,.
\end{equation}
The dimensionless Hubble parameter is
\be
h(z)=\frac{H(z)}{H_0}=(1+z)^{1/\a}.
\label{eq:dimensionless_hubble}
\end{equation}

\subsubsection{Present-day scale factor}

\vspace{-0.1in}
We define the present `radius' of the universe (\ref{eq:ansatz}) as
\be
a_0 =B\fr{c}{H_0}\,\,.
\label{eq:a_0}
\end{equation}
\subsubsection{Angular diameter distance }

\vspace{-0.2in}
There are many ways to define a distance in cosmology---parallax distance, 
angular diameter distance, luminosity distance, proper motion distance, etc
(see~\ref{sec:distance}). It is the angular diameter distance that is relevant
to the angular separation of images. 
 
Consider a source at $r=r_1$ which emitted light at $t=t_1$. The
observed angular diameter of the source, $\delta$, is related to
the proper diameter of the source, D, by
\be
\delta = \fr{D}{a(t_1)\,r_1}\,\,.
\end{equation}
The angular diameter distance $\rm D_A$ is defined to be 
\be
{\rm D_A}(z) = \fr{D}{\d}= a(t_1)\,r_1 = \frac{a_0 r_1}{1+z},
\label{eq:D_A_definition}
\end{equation}
where $r_1(z)$ is the coordinate distance to a redshift $z$. Angular
diameter distance of a source at $z_2$ measured by an (fictitious) observer at
$z_1$ is given by \be
D_{\rm A}(z_1,z_2) = \fr{a_0 r_{12}}{1+z_2}\,\,.
\label{eq:z_12}
\end{equation}
Light travels on
null geodesics, $ds^2=0$. If a comoving observer is at coordinates 
$(r_0,\theta_0,\phi_0)$ at time $t_0$, the geodesics intersecting 
$r_0=0$ are lines of constant $\t$ and $\phi$. Geodesic equation becomes
\be
0=cdt^2-a^2(t) \frac{dr^2}{(1+r^2)}
\end{equation}
and the light signal emitted from coordinates $(r_1,\t,\phi)$ at time
$t$ will reach the observer at time $t_0$ determined by
\be
\int_{t}^{t_0} \frac{c\,dt'}{a(t')} = \int^{r_1}_0
\frac{dr}{\sqrt{1+r^2}}
\label{eq:over_r}
\end{equation}
We can convert the integrals over $t$ into integrals over $z$ by
differentiating (\ref{eq:redshift}),  
$$
\frac{dz}{dt} = -\frac{a_0}{a^2} 
\dot{a}=-\frac{a_0}{a}\frac{\dot{a}}{a} = -(1+z)H(z)\,\,,
$$
to obtain
\be
dt=-\frac{dz}{(1+z) H(z)}\,\,.
\label{eq:dt}
\end{equation}
Thus, equation (\ref{eq:over_r}) becomes:
\be
\int_{0}^{z}\frac{c\,dz}{H(z)(1+z) a} = \int_{0}^{r_1}
\frac{dr}{\sqrt{1+r^2}}
\end{equation}
Since $a_0/a=1+z$, we use it to obtain
\be
\frac{c}{a_0}\int_{0}^{z_1}\frac{a_0\,dz}{H(z)(1+z) a} =
\frac{c}{a_0}
\int_{0}^{z_1}\frac{dz(1+z)}{H(z)(1+z)}=\frac{c}{a_0}\int_{0}^{z_1}
\frac{dz}{H(z)}\,\,,
\end{equation}
or, in terms of a dimensionless Hubble parameter $h(z)$,
Eq.~\ref{eq:over_r}
becomes
$$
\frac{c}{H_0 a_0}\int_{0}^{z_1}\frac{dz}{h(z)} =
\int_{0}^{r_1}\frac{dr}{\sqrt{1+r^2}}\,\,.
$$

\SS{Comoving Coordinate Distance $r$}

For an open universe, $k=-1$, and we obtain
$$
\frac{c}{H_0 a_0}\int_{0}^{z_1}\frac{dz}{h(z)} = \sinh^{-1}{r_1}\,\,.
$$
Thus, 
$$
r_1=\sinh{\left[\fr{c}{H_0a_0}\int_0^{z_1}\fr{dz}{h(z)}\right]}\,\,.
$$

\vspace{-0.3in}
\SS{$D_{\rm A}$ formulae}
If we take the value of $a_0$ from Eq.~\ref{eq:a_0}, 
we obtain the following value of $r_1$:
\be
r_1=\sinh{\left[\fr{1}{B}\int_0^{z_1}\fr{dz}{h(z)}\right]}\,,
\end{equation}
And the expression for $D_{\rm A}$ is:
\be
D_{\rm A}(z,\a)= \fr{Bc}{(1+z)H_0}\sinh{\left[ 
\fr{1}{B} \int_0^{z_1} \fr{dz}{h(z)}\right]}\,,
\end{equation} 
with the integral 
$$
\int_0^{z_1}\fr{dz}{h(z)} = \fr{\a}{\a -1} \left\{(1+z)^{\fr{\a -a}{\a}}-
1^{\fr{\a -1}{\a}} \right\}\,\,.
$$
Finally, distance formula is
\be
D_{\rm A}(z,\a) = \fr{Bc}{(1+z)H_0}
\sinh{\left[ \fr{1}{B}\frac{\a}{\a-1} 
\left\{ (1+z)^{\frac{\a-1}{\a}} - 1^{\frac{\a-1}{\a}} \right\}
\right]}\,\,.
\label{eq:D_A}
\end{equation}
The distance between two different redshifts is:
\be
D_{\rm A}(z_1,z_2 ,\a) = \fr{Bc}{(1+z_2) H_0}
\sinh{\left[ \fr{1}{B}\frac{\a}{\a-1}
\left\{ (1+z_2)^{\frac{\a-1}{\a}} - (1+z_1)^{\frac{\a-1}{\a}} 
\right\} \right]}\,\,.
\end{equation} 

\SS{Limiting ($\a \rightarrow 1$) formulae}

We know that  $h(z)=(1+z)^{1/\a}$, with $\a \rightarrow 1$, thus,
$h(z)=(1+z)$,
then the integral 
\be
\int_{0}^{z}\fr{dz'}{1+z'} = \ln{(1+z)}\,\,,
\end{equation}
and the Eq.~\ref{eq:D_A} reduces to
\be
{\rm D_A}(z) = \fr{Bc}{H_0} \fr{1}{1+z}
\sinh{\left[\fr{1}{B}\ln{(1+z)}\right]}=
\fr{Bc\left[(1+z)^{2/B} - 1\right]}{2\,H_0(1+z)^{\fr{B+1}{B}}}\,\,.
\end{equation}
The distance between two redshifts is, accordingly,
\be
{\rm D_A}(z_1,z_2) = \fr{Bc}{2 H_0}\fr{\left[(1+z_2)^{2/B} -
(1+z_1)^{2/B} \right]}{(1+z_1)^{1/B}(1+z_2)^{\fr{B+1}{B}}}\,\,.
\end{equation}

\subsubsection{Look-back time}

The look-back time, $\Delta t=|t-t_0|$, is the difference between the age of
the universe when a particluar light ray was emitted and the age of the
universe now: \be
\Delta t(a;a_0)=\int_{a}^{a_0}\fr{da}{\dot{a}(a)}\,\,\,.
\end{equation}
We can obtain the expression for the look-back time  from Eq.~\ref{eq:dt} and
Eq.~\ref{eq:dimensionless_hubble}. Since we define $t_0$ as zero and time is
increasing  as we look back, we drop the negative sign in that expression.
Thus,
\be
\fr{dt}{dz}=\fr{1}{H_0 (1+z)^{\fr{\a +1}{\a}}}\,\,,
\end{equation}
and finally the expression we seek is:
\be
\fr{c\,dt}{dz_{\rm L}}=\fr{c}{H_0 (1+z_{\rm L})^{\fr{\a
+1}{\a}}}\,\,. 
\label{eq:backtime}
\end{equation}    

\subsection{Basic equations of gravitational lensing statistics}

Given a lens model, the number counts of galaxies--lenses and the properties
of the lenses, we compute the probability $p_i$ that quasar $i$ is lensed and
the probability $p_i(\D\t_i)$ that quasar $i$ is lensed and has image
separation $\D\t_i$.  We shall consider only early types of galaxies,
elliptical and lenticulars, E/S0, neglecting the contribution of spirals as
lenses. This is because the velocity dispersion $v$ of spirals is small
compared to E/S0 galaxies, outweighing the larger number density. The numbers
of E/S0 and spirals are roughly 30\% and 70\%, respectively, whereas in our
adopted sample the velocity dispersion of ellipticals is about 200 km s$^{-1}$
and that of spirals is about 130 km s$^{-1}$ \cite{Loveday}. The calculations
for the lensing statistics depend strongly on this quantity, since the lensing
optical depth goes as the fourth power of the velocity dispersion (see
Eq.~\ref{eq:F*}).  

It is increasingly clear \cite{K96} that E/S0 galaxies are effectively
singular. The almost uniform absence of central images in the observed lenses
and models of individual lenses imply core radius smaller than 100 $h^{-1}$
pc and essentially suggesting that the galaxy lenses are nearly singular
\cite{Wallington93,K95}. We will model the lensing galaxies as singular ($=$
zero core radius) isothermal spheres (SIS). The detailed lensing properties of
singular isothermal spheres are described in Section~\ref{sec:SIS}. Here we
simply state the most important relations for the present calculations. A SIS
lens with a velocity dispersion $v$ at a redshift $z_{\rm L}$ will produce two
images of a quasar at a redshift $z_{\rm S}$ separated by an angle $\D\t$ 
\be
\D\t = 2 \a_{\rm d} \fr{D_{\rm LS}}{D_{\rm S}}\,\,,
\label{eq:separation}
\end{equation}
if angular position of the source is less than the critical angle $\b_{\rm
cr} \equiv \a_{\rm a} D_{\rm LS}/D_{\rm S}$. The deflection angle, $\a_{\rm
d}$, is given for all impact parameters to be 
\begin{equation}
\a_{\rm d} = 4\pi \left(\fr{v}{c}\right)^2\,\,.
\label{eq:defangle}
\end{equation}
The angular separation of the two images is independent of the impact parameter
as long as it is small enough to produce two images. The critical impact
parameter is defined by $a_{\rm cr} \,\equiv \, D_{\rm L} \b_{\rm cr}$ or, with
the help of the previous definitions,
\begin{equation}
a_{\rm cr}=4\pi \left( \fr{v}{c} \right)^2 \fr{D_{\rm L}D_{\rm LS}}{D_{\rm S}}\,\,.
\end{equation}
The quasars are treated as point sources of radiation. We assume that
no evolution of galaxies or quasars with cosmic time (quasar evolution is
irrelevant, since the quasar redshift distribution will be drawn from observed
samples). In other words, the comoving number density of lenses is 
conserved
\be
n_{\rm L} = n_0 (1+z_{\rm L})^3\,\,,
\label{eq:n_L}
\end{equation} 
where $n_0$ is an average comoving density measured at the present epoch.
Merging between galaxies and infall of surrounding mass onto galaxies are two
posible processes that can change the comoving density of galaxies and/or
their mass. Under the generic relation between the velocity dispersion and
mass of early-type galaxies, Rix et al \cite{rix} and Mao\&Kochanek
\cite{mao} found that merging and/or evolution do not significantly change
the statistics of lensing. 

\vspace{-0.3in}
\subsubsection{Cross-section and optical depth of lensing.}

The cross-section $\s$ for "strong" lensing events is given by$\s = \pi
a_{\rm cr}^2$. Using (\ref{eq:defangle}) and the definitions from the
previous subsection, we write the cross-section as
\be
\s = 16 \pi^3 \left(\fr{v}{c}\right)^4 \left(\fr{D_{\rm L}D_{\rm LS}}{D_{\rm S}}
\right)^2\,\,.
\end{equation} 
Looking at this equation we see that the cross-section is largest approximately
halfway in the distance between the source and the observer; and $\s$ vanishes
at the two endpoints. To find the average effect on an image passing within 
$a_{\rm cr}$ of a mass (``scoring a hit"), we average over the cross-section to
find the mean image separation as
\be
\overline{\D \t} = 8\pi \left(\fr{v}{c}\right)^2 \fr{D_{\rm LS}}{D_{\rm S}}\,\,.
\end{equation}
The differential probability (or the optical depth) $d\tau$ that a line of sight
intersects a galaxy-lens at $z_{\rm L}$ in traversing the path of $dz_{\rm
L}$ from a population with number density $n_{\rm L}$ is given by a  ratio of
differential light travel distance $cdt$ to its mean free path between
successive encounters with galaxies, $1/n_{\rm L}(z)\s$, 
\be
d\tau=n_{\rm L}(z)\s\fr{cdt}{dz_{\rm L}}dz_{\rm L}\,\,.
\end{equation}
For our case $n_{\rm L}(z)$ is given by (\ref{eq:n_L}) and the quantity 
$ cdt/dz_{\rm L}$ is obtained in the previous section (Eq.~\ref{eq:backtime}). 
Substituting for $\s$ and $n_{\rm L}(z)$, we get
\be
d\tau = \fr{16\pi^3}{c^4}(1+z_{\rm L})^3 \la n_0v^4 \ra 
\left(\fr{D_{\rm L} D_{\rm LS}}{D_{\rm S}}\right)^2\fr{cdt}
{dz_{\rm L}}dz_{\rm L}\,\,.
\label{eq:dtau}
\end{equation}

Assuming that the brightness distribution of galaxies at any given redshift is 
described by a Schechter function, the comoving density of galaxies at
redshift $z$ and with luminosity between $L$ and $L+dL$ is
\be
\P(L,z) dL = n_{*}(z) \left( \fr{L}{L_{*}(z)} \right)^{\hat \a} 
\exp{\left( -\fr{L}{L_{*}(z)} \right)} \fr{dL}{L_{*}(z)}\,\,.
\label{eq:lumfunz}
\end{equation}
The parameter $n_{*}(z)$ is the average comoving density, 
$L_{*}(z)$ is the characteristic luminosity at which the luminosity function
exhibits a rapid change in the slope ($\log{n},\,\log{L}$)-plane and $\hat \a$ 
gives the slope of the luminosity function in the ($\log{n},\,\log{L}$)-plane,
when $L \ll L_{*}$. The comoving number density of galaxies, characteristic
luminosity and mass of a galaxy at any redshift remain constant, therefore,
$n_{*}(z) = n_{*}(0) = \mbox{constant}$ and $L_{*}(z) = L_{*}(0) =
\mbox{constant}$. ``0" refers to present-day values. This is the most
commonly used luminosity function of early type galaxies. Thus,
Eq.~\ref{eq:lumfunz} becomes \be
\P(L,z=0)\,dL = n_{*} \left( \fr{L}{L_{*}} \right)^{\hat \a} 
\exp{\left( -\fr{L}{L_{*}} \right)} \,\fr{dL}{L_{*}}\,\,.\,
\label{eq:lumfun}
\end{equation}
where $n_{*}$, $\hat \a$ and $L_{*}$ are the normalization factor, index of the
faint-end-slope and the characteristic luminosity at the present epoch, 
respectively. These values are fixed in order to fit the current luminosities and
densities of galaxies. From Eq.~\ref{eq:dtau} and Eq.~\ref{eq:lumfun} we have
\be
\la n_0 v^4 \ra =  v_{*}^4 n_{*} \int_0^{\infty}
\left( \fr{L}{L_{*}} \right)^{\hat \a} \exp{\left( -\fr{L}{L_{*}} \right)}\, 
\fr{dL}{L_{*}} \left( \fr{v}{v_{*}} \right)^4 \,.
\label{eq:n_0}
\end{equation}  
    We assume the velocity dispersion $v$ is related to the luminosiy $L$ by
the empirical Faber-Jackson relation for E/S0 galaxies:
\be
\left(\fr{L}{L_{*}}\right) = \left( \fr{v}{v_{*}}\right)^{\g}\,\,.
\label{eq:F-J}
\end{equation}
Therefore, Eq.~(\ref{eq:n_0}) becomes 
\be
\la n_0 v^4 \ra =  v_{*}^4 n_{*} \int_0^{\infty}
\left( \fr{L}{L_{*}} \right)^{4\hat \a +\g} \exp{\left( -\fr{L}{L_{*}}
\right)}  \fr{dL}{L_{*}} \,\,.
\end{equation} 
By integrating it over the luminosity function at redshift $z$, we obtain the 
differential probability 
\be 
d\tau=\fr{16 \pi^3}{c^4} (1+z_{\rm L})^3 n_{*}v_{*}^4 \G \left(
\hat \a +\fr{4}{\g} +1 \right) \left(\fr{D_{\rm L} D_{\rm LS}}{D_{\rm
S}}\right)^2 \fr{cdt}{dz_{\rm L}}dz_{\rm L}\,\,
\end{equation}
where $\G$ is the normal gamma function.

\vspace{-0.2in}
\subsubsection{Image separation statistics}

We will now present the calculations of the statistics of angular separation
between the two outer images. If we define the `dimensionless' image splitting
as $\phi = \D \t/8\pi \left(v_*/c\right)^2$, we can find the differential
optical depth of lensing in traversing $dz_{\rm L}$ with the angular
separation between $\phi$ and $\phi +d\phi$ as $\fr{d^2\tau}{dz_{\rm L}d\phi}
d\phi dz_{\rm L}$. From (Eq.~\ref{eq:separation}) and luminosity-velocity
relation (Eq.~\ref{eq:F-J}), we obtain the relation \be
\fr{L}{L_{*}}=\left(\fr{D_{\rm S}}{D_{\rm LS}}\phi \right)^{\g/2}\,\,.
\end{equation}
Taking the differential,
\be
\fr{dL}{L_{*}}=\fr{\g}{2}\left(\fr{D_{\rm S}}{D_{\rm LS}}\phi\right)^{\g/2}
\fr{d\phi}{\phi}\,\,.
\label{eq:lum-vel}
\end{equation}
Returning to (Eq. 1.54), we write $d\tau/dz_{\rm L}$ as
\be
\fr{d\tau}{dz_{\rm L}}=n_{\rm L}(z)\fr{16\pi^3}{c^4}v^4\left(\fr{D_{\rm L}
D_{\rm LS}}{D_{\rm S}}\right)^2\fr{cdt}{dz_{\rm L}}\,\,.
\end{equation}
The differential optical depth of lensing in traversing $dz_{\rm L}$ with
the angular separation between $\phi$ and $\phi +d\phi$ is
\berr
&&\hskip -0.8in \int_0^{\infty}\fr{d^2\tau}{dz_{\rm L}d\phi}d\phi= \no \\
&& \\
&& n_{*}v_{*}^4 \int_0^{\infty}\left(\fr{L}{L_{*}}\right)^{\hat \a}
\exp{\left(-\fr{L}{L_{*}}\right)}\fr{dL}{L_{*}}\left(\fr{L}{L_{*}}\right)^{4/\g}
\left(1+z_{\rm L}\right)^3\fr{16\pi^3}{c^4} 
\left(\fr{D_{\rm L}D_{\rm LS}}{D_{\rm S}}\right)^2 \fr{cdt}{dz_{\rm L}}\,\,.\no
\err
Using the relations (Eq.~\ref{eq:lum-vel}), we obtain
\berr
\hspace{-1 cm}\lefteqn{\fr{d^2\tau}{dz_{\rm L}d\phi}d\phi dz_{\rm L}=}\no \\
&& \\
&&\hspace{-0.7 cm}F^{*}(1+z_{\rm L})^3\fr{H_0}{c}
\fr{\g/2}{\G \left(\hat \a +1+\fr{4}{\g}\right)}\fr{cdt}{dz_{\rm L}}
\left(\fr{H_0 D_{\rm L}D_{\rm LS}}{c\,\, D_{\rm S}}\right)^2
\left(\fr{D_{\rm S}}{D_{\rm LS}}\phi\right)^{\fr{\g}{2}(\hat \a +1+\fr{4}{\g})}
\exp{\left[\left(-\fr{D_{\rm S}}{D_{\rm LS}}\phi \right)^{\fr{\g}{2}}\right]}
\fr{d\phi}{\phi}dz_{\rm L}\,. \no
\label{eq:d2tau}
\err
Here we introduced the useful dimensionless quantity $F^*$ which
measures the effectiveness of matter in producing multiple images \cite{TOG}
\begin{equation}
F^{*} \equiv \fr{16\pi^3}{cH_0^3}n_*v_*^4\G \left(\hat \a
+1+\fr{4}{\g}\right)\,\,. \label{eq:F*}
\end{equation}

\subsubsection{Lens and source parameters.}   
The variables relating galaxy numbers counts and the isothermal lens model
are the number density of E/S0 galaxies $n_{*}$; the Schechter function slope 
$\hat \a$; the Faber-Jackson exponent $\g$; and the velocity dispersion of the
dark matter for an $L_{*}$ galaxy $v_{*}$. The Schechter function slope
$\hat \a$ controls the relative number of low- and high-mass galaxies. We use
the following list of lens parameters for our calculations \cite{Loveday}:
\begin{center}
\begin{tabular}{|c|ccccc|}\hline\hline
$Survey$ & $ \alpha$ & $ \gamma$ & $ v^{*} (Km /s)$ & $\phi^{*}
(Mpc^{-3})$ & $ F^{*}$
\\ \hline
\hline
$LPEM$ & $+ 0.2$ & $4.0$ &$205$ &$3.2 \times 10^{-3}$& $0.010$   \\
\hline
\end{tabular}
\end{center}
We consider a sample of 867 ($z > 1$) high luminosity optical quasars which
include 5 lensed quasars ($1208 +1011$,  H $1413+117$, LBQS $1009+0252$, PG
$1115+080$, $0142+100$). This sample  is taken from optical lens surveys, such
as the HST Snapshot survey, the Crampton survey, the Yee survey, Surdej
survey, the NOT Survey and the FKS survey \cite{surveys}. The lens surveys and
quasar catalogues usually use V magnitudes, so we transform $m_{V}$ to a
B-band magnitude using $B-V=0.2$ \cite{Bahcall}. 

We make two corrections to the optical depth to get the lensing probability:
magnification bias and selection function.

\vspace{-0.8in}
\paragraph{Magnification bias. }
Lensing increases the apparent brightness of a quasar causing 
over-representation of multiply images quasars in a flux-limited sample. This
effect is called {\emph magnification bias}. It is an enhancement of the
probability that a quasar is lensed, that is why we have to include this
correction in the probability function. The bias for a quasar at a redshift
$z$ with apparent magnitude $m$ is given as \cite{fukugita,K93,K96}
\be
B(m,A_{\rm lim},A_2,z)=\left(\fr{dN(m.z)}{dm}\right)^{-1}
\int_{A_{\rm lim}}^{A_2}\fr{dN(m_{\rm A},z)}{dm} p(A)dA\,\,.
\end{equation}
Here $A$ is the total magnification, $A_{\rm lim}$ the magnification 
at which the images have the minimum detectable flux ratio (for 
a SIS model, $A_{\rm lim}=A_0=2$), $m_{\rm A}=m+2.5\log{A}$ is the lensing
enhanced magnitude and $p\,(>A)$ is the probability distribution for 
the two images having a total magnification larger than $A$, $p(A)=8/A^3$
for a SIS model. We can allow the upper limit on magnification $A_2$ 
to be infinite, but in practice we set it to be $A_2=10^4$. For the quasar
apparent magnitude number counts we use Kochanek's broken power law
\cite{K96}  
\be
\fr{dN(m,z)}{dm} \propto \left(10^{-a(m-m_0(z))} + 
10^{-b(m-m_0(z))}\right)^{-1}\,\,,
\end{equation}
where the bright-end slope index $a$ and faint-end slope index $b$ are
constants and the break magnitude $m_0$ evolves with redshift as
$$
m_0(z)=
\left\{
\barr{lcl}
m_0+(z+1)  & \mbox{if} & z<1 \\
m_0        & \mbox{if} & 1<z<3\\
m_0-0.7(z-3) & \mbox{if} & z>3\,\,.
\earr
\right.
$$
Fitting this model to the quasar luminosity function data in \cite{Hartwich}
for $z>1$, Kochanek finds that the `best model' has $a=1.07$, $b=0.27$ and
$m_0=18.92$ at B magnitude. Thus, magnitude corrected probability $p_i$ for
the quasar $i$ with  apparent magnitude $m_i$ and redshift $z_i$ to get lensed
is $p_i=\tau(z_i) B(m_i,A_{\rm lim},A_2,z_i)$.

\vspace{-0.4in}
\paragraph{Selection function. }
Selection effects are caused by limitations on dynamic range, limitations on
resolution and presence of confusing sources such as stars. In SIS model
the selection function is modeled by a maximum magnitude difference $\D m(\t)$
that can be detected for two images separated by $\D \t$. This is equivalent
to a limit on the flux ratio between two images $f=10^{0.4 \D m(\t)}$. The
total magnification becomes $A_f=A_0(f+1)/(f-1)$. So, the survey can only
detect lenses with magnifications greter than $A_f$. This sets the lower
limit on magnifications and in the bias function $A_{\rm lim}$ gets replaced
by $A_f$. To get selection function corrected probabilities, we divide our
sample into two parts: the ground based surveys and the HST Snapshot survey and
use the selection function for each survey as suggested by Kochanek
\cite{K93}. 

The corrected lensing probability and image separation distribution function
for a single source at redshift $z_{\rm S}$ are given as \cite{K96}
\be
p^{'}_{i}(m,z) = p_{i}\int \frac{ d(\Delta\theta)\,
p_{c}(\Delta\theta)\emph{B}(m,z,M_{f}(\Delta\theta),M_{2})}
{\emph{B}(m,z,M_{0},M_{2})},
\label{prob2}
\end{equation}
and
\be
p^{'}_{ci} =p_{ci}(\Delta\theta)\,\frac{p_{i}}{p_{i}^{'}}\,
\frac{\emph{B}(m,z,M_{f}(\Delta\theta),M_{2})}
{\emph{B}(m,z,M_{0},M_{2})}\,\,,
\label{confi}
\end{equation}
where
\be
p_{c}(\Delta\theta) =
\frac{1}{\tau(z_{S})}\,\int_{0}^{z_{S}}\frac{d^{2}\tau}{dz_{L}d(\Delta\theta)}
\,dz_{L}\,\,.
\label{pcphi}
\end{equation}
Equation (\ref{confi}) defines the configuration probability. It is the
probability that the lensed quasar $i$ is lensed with the observed image
separation.
 
\subsection{Testing the model against observations}
 
The above basic equations were used to perform the following test:
\begin{trivlist}
\item The sum of the lensing probabilities $p_{i}^{'}$ for the optical 
QSOs gives the expected number of lensed quasars, $n_{\rm L} = \sum\,
p_{i}^{'}$. The summation is over the given quasar sample. We look for those
values of the parameter for which the adopted optical sample has exactly five
lensed quasars (that is, those values of the parameters for which $n_{\rm
L}=5$). 

We started with a two parameter fit. We allowed $\a$ to vary in the range ($0.0
\leq \a \leq 2.0$) and $B$ to vary in the range ($0.5\leq B \leq 10.0$). We
observe that for $B\ge 1$, $D_A$ becomes independent of it (as is also
obvious from equation (\ref{eq:D_A})). In the previous works constraining
power law cosmology \cite{annu,abha}, the value of $B = 1$ was found to be
compatible with the observations. Incidentally, we can estimate the present
scale factor of the universe as $a_0 \approx c/H_0$.  Therefore, we used $B =
1$ in further analysis.     

Fig.~\ref{fig:NlA} shows the predicted number of lensed quasars for the above 
specified range of $\alpha$. We obtained $n_{L} = 5$ for $\a = 1.06$. We
further generated $10^{4}$ data sets using bootstrap method (see description in
\cite{abhathesis}) and found the best fit for $\a$ for each data set in order
to obtain error bars on $\a$. We finally obtained $\a = 1.09 \pm 0.3$.

\begin{figure}[ht]
\vspace{-1.3in}
\centerline{
\epsfig{figure=chapter4/Nl-alpha.ps,width=1.\textwidth}}
\vspace{-5.2in} 
\caption{Predicted number of lensed quasars $n_{\rm L}$ in the adopted optical
quasar sample, with  $\Delta\theta \leq 4''$, vs. power index $\a$.}
\label{fig:NlA} 
\end{figure}
\end{trivlist}

The maximum likelihood analysis was also performed \cite{abhathesis} to
determine the value of $\alpha$, for which the observed sample becomes the
most probable observation. It was found that $0.85 \leq \a \leq 1.56$ at
$1\sigma$  ($68\%$ confidence level), and $0.65 \leq \a \leq 2.33$ at $2\sigma$
($95.4\%$ confidence level). It is also interesting to notice that for a
general power law cosmology the simplest constraint on $\a$ comes from the
relation $\a=H_0 t_0$ (Eq.~\ref{eq:exact}). With updated value of $H_0=70
\pm7$ km/sec/Mpc \cite{Freedman00} and $t_0=14\pm2$ Gyr \cite{pont}, this
constraint gives $\a=0.98 \pm 0.25$. 

\section{Conclusions}

In this section we discussed the general power law cosmology and the ways to
constraint its power index. We have derived angular diametere distances for
this cosmology. We described the general formulation of the gravitational
lensing statistics and used it to constraint the parameters for that
cosmology. These results together with other tests were used in \cite{rita4}
in the combined form and the conclusion made was that open linear coasting
cosmology is not ruled out by the present observations.  















 







   




